Numerical simulation of endovascular treatment options for cerebral aneurysms

Predicting the long-term success of endovascular interventions in the clinical management of cerebral aneurysms requires detailed insight into the patient-specific physiological conditions. In this work, we not only propose numerical representations of endovascular medical devices such as coils, flow diverters or Woven EndoBridge but also outline numerical models for the prediction of blood flow patterns in the aneurysm cavity right after a surgical intervention. Detailed knowledge about the post-surgical state then lays the basis to assess the chances of a stable occlusion of the aneurysm required for a long-term treatment success. To this end, we propose mathematical and mechanical models of endovascular medical devices made out of thin metal wires. These can then be used for fully resolved flow simulations of the post-surgical blood flow, which in this work will be performed by means of a Lattice Boltzmann method applied to the incompressible Navier-Stokes equations and patient-specific geometries. To probe the suitability of homogenized models, we also investigate poro-elastic models to represent such medical devices. In particular, we examine the validity of this modeling approach for flow diverter placement across the opening of the aneurysm cavity. For both approaches, physiologically meaningful boundary conditions are provided from reduced-order models of the vascular system. The present study demonstrates our capabilities to predict the post-surgical state and lays a solid foundation to tackle the prediction of thrombus formation and, thus, the aneurysm occlusion in a next step.

==> PM_LBM.tex <==
Within the description of (wall) boundary conditions we already mentioned that our medical device-models (see Section~\ref{sec:DeviceModelling} and \ref{sec:NumericalSimulations}) can be immersed into the blood-stream as obstacles with velocity Dirichlet data $\vel=\Vec{0}$ on their boundary. This approach uses the precise geometry information about the inserted devices, however, therefore it also requires a resolution fine enough to resolve all those (filigree) geometrical features, where especially the endovascular devices we are dealing with are full of. The approach we are discussing within this section now takes a different route and will eventually act as a surrogate model for those fully resolved e.g. coiling-devices, also allowing for coarser resolutions.

\subsubsection{Porous medium modelling and homogenization} \label{subsubsec:PorousFlowModelling}
The fundamental idea of the model discussed in this section is to actually \textit{not} fully resolve the medical device, but actually to completely replace it by means of a porous volumetric region. Within this region two spatial fields, a scalar porosity $\porosity(\vec{x})\in [0,1]$ as well as a positive definite, but potentially anisotropic permeability tensor $\tens{K}(\Vec{x})\in\R^{3\times 3}_{\textup{sym}}$ constitute the porous material with their (inhomogeneous) distribution trying to resemble the structure of the originally placed medical device, best to be imagined as a diffuse ``shadow'' of its geometry. The presence of this {\PM} can be accounted for within the fluid-mechanical equations in a ``minimal-invasive'' way by modifying the momentum equation \eqref{eq:NavierStokes1} of the Navier-Stokes system according to \cite{nithiarasu1997natural} to become:
\begin{equation}\label{eq:PM_NavierStokes}
    \frac{\partial\vel}{\partial t}+\left(\vel\cdot\grad\right)\left(\frac{\vel}{\porosity}\right)+\frac{1}{\den}\grad\left(\porosity \p\right)-\grad\cdot\left(2\frac{\vis_e}{\den}\tens{\epsilon}(\vel)\right)=\vec{F}=-\frac{\porosity \vis}{\den}\tens{K}^{-1}\vel-\porosity F_{\porosity}\tens{K}^{-1/2}\|\vel\|_2\vel.
\end{equation}
I.e. in addition to the porosity scaling on the left-hand-side, the equation way mainly changed by adding additional force-contributions to the right-hand-side. Within this equation the first of these terms on the right hand side is a force contribution due to Darcy's-law, the second, nonlinear one a so called Forchheimer-term with the geometric function $F_{\porosity}=1.75/\sqrt{150\,\porosity^3}$ \cite{guo2002lattice}. This model has already been successfully employed also for other applications such as porous ground-water flow in \cite{benamram2016field} or in the context of phase-change heat transfer in \cite{he2019lattice}.

\bw{Another way to ...}

\paragraph{Homogenization} If we now aim for replacing a fully resolved medical device-geometry such as a coil, being the final result of our coil-deployment simulation (see Section~\ref{subsec:Coils}), by means of a porous medium, we are faced with the challenge to derive suitable porosity and permeability fields that actually resemble in a somewhat diffused way the original geometry. To reach this goal we employ a homogenization procedure similar to \cite{romero2023modeling}, where for each spatial point of interest $\vec{x}$, e.g. the cell-centers in our computational grid, a local \textit{representative elementary volume} (REV) is build as a cube of edge length $a$ around $\Vec{x}$. Then, within this cube the volume fraction of space \textit{not} occupied by the coiling-device, i.e. pore-space, divided by the total volume of the cube is formed yielding a measure of \textit{local} porosity $\porosity(\Vec{x})$. By adapting the REV size $a$ it is also possible to steer the resolution level of the resulting porosity field from being strongly contrasted in case of small $a$ towards nearly completely homogeneous for large $a$.\\
\indent With the question for the  porosity field being solved, we still have to derive a (tensorial) permeability field $\tens{K}(\Vec{x})$ as well. In the present work we therefore employ the Kozeny-Carman relation as in \cite{guo2002lattice}, i.e.
\begin{equation*}
    K(\Vec{x})=\frac{\porosity(\Vec{x})^3d_t^2}{150(1-\porosity(\Vec{x}))^2}
\end{equation*}
with $d_t$ being the device's (wire)thread diameter, also see \cite{schulz2019beyond} \tum{Natalia: Can you please check this again, which one exactly was used} to derive $\tens{K}(\Vec{x})=\textup{diag}(K(\Vec{x}),K(\Vec{x}),K(\Vec{x}))$, hence actually only scalar permeability $K(\Vec{x})$, locally depending on the porosity $\porosity(\Vec{x})$. A way to utilize the directivity information of the inserted wire to obtain an \textit{orthotropic} permeability tensor will be discusses in a separate publication, currently in preparation; see our research webpage\footnote{Research-webpage at TUM: \url{http://go.tum.de/696501}} for a list of regularly updated publications about this topic.

\begin{figure}
\begin{center}
\includegraphics[height=5cm]{images/Porosity_GAMM.png}\hspace{1cm}\includegraphics[height=5cm]{images/Porosity_GAMMn.png}\hspace{5mm}\includegraphics[width=1.8cm]{images/CBAR_porosity.png}
\end{center}
\caption{(Section of) the porosity field $\porosity(\Vec{x})$ obtained from homogenization within the aneurysm. \textbf{(left)} Porosity field together with the coil-structure used for the homogenization. \textbf{(right)} Same porosity field, but without the coil. Its (very rough) position can still be guessed from its ``porous medium shadow''. \label{fig:StentModel}}
\end{figure}

\subsubsection{Porous medium treatment within Lattice Boltzmann methods} \label{subsubsec:PorousFlowLBM}

Similar to the assumption of constant viscosity, in our {\LBM} introduction Section~\ref{subsubsec:FreeFlowNumericalTreatmentLBM} we have initially assumed external forces $\vec{F}$ to be zero. While this (neglecting gravity) is true within any free-flow region of our fluid-mechanical problem, in \eqref{eq:PM_NavierStokes} the presence of the {\PM} is modelled via a non-vanishing, but actually velocity dependent body force. Various forcing schemes have been developed for {\LBM} in order to deal with such force contributions, while especially for the presented case the authors of \cite{guo2002lattice} have given the correct modifications of \eqref{eq:LBMUpdate} and \eqref{eq:DiscrMacroQuant} to incorporate the influence of the {\PM}. The main change is the additional term:
\begin{equation*}
    \Delta tF_i=\Delta tw_i\rho\left(1-\frac{1}{2\tau}\right)\left(\frac{\Vec{c}_i\cdot \vec{F}}{c_s^2}+\frac{(\vel\Vec{F}^{\top}):\left(\Vec{c}_i\Vec{c}_i^{\top}-c_s^2I\right)}{\phi c_s^4}\right)
\end{equation*}
that gets added to the right hand side of \eqref{eq:LBMUpdate} as well as the force-corrected velocity expression:
\begin{equation}\label{eq:PMVelCorrection}
    \rho\vel=\sum_{i=0}^{n-1}\vec{c}_if_i+\frac{\Delta t}{2}\rho\Vec{F}
\end{equation}
replacing \eqref{eq:DiscrMacroQuant}. It should be noted that due to the velocity dependent form of $\Vec{F}$ according to \eqref{eq:PM_NavierStokes}, \eqref{eq:PMVelCorrection} is a non-linear equation in $\vel$. Fortunately, it is only quadratic in $\vel$ and hence can be solved explicitly with detailed steps being listed again in \cite{guo2002lattice}. This, now modified, {\LBM} realizes a one-domain approach for the treatment of the {\PM} to free-flow coupling, simply by modifying the porosity parameter $\porosity(\Vec{x})$ to attain a value of (close to) $1$, where free-flow is supposed to begin and a value within $[0,1)$ where a {\PM} is supposed to reside, with its concrete value stemming for example from the homogenization algorithm. In the presented application of {\CAs} the typical situation will be a {\PM} inside the sack of the aneurysm modelling the presence of a coiling-device, and free-flow within the adjacent vessel outside the aneurysm, see e.g. Fig.\,\ref{fig:TBA} in Section~\ref{sec:NumericalSimulations}.
